Reduced order methods for parametrized non-linear and time dependent optimal flow control problems, towards applications in biomedical and environmental sciences

We introduce reduced order methods as an efficient strategy to solve parametrized non-linear and time dependent optimal flow control problems governed by partial differential equations. Indeed, the optimal control problems require a huge computational effort in order to be solved, most of all in physical and/or geometrical parametrized settings. Reduced order methods are a reliable and suitable approach, increasingly gaining popularity, to achieve rapid and accurate optimal solutions in several fields, such as in biomedical and environmental sciences. In this work, we employ a POD-Galerkin reduction approach over a parametrized optimality system, derived from the Karush-Kuhn-Tucker conditions. The methodology presented is tested on two boundary control problems, governed respectively by (i) time dependent Stokes equations and (ii) steady non-linear Navier-Stokes equations.

==> 2_Problem_Maria.tex <==
%\subsection{Linear Quadratic Time Dependent \ocp s}
%\label{Maria_Problem}
%We briefly introduce the theoretical framework of linear quadratic time dependent \ocp s, i.e. \ocp s governed by a time dependent state equation based on the minimization of a quadratic cost functional.  The mathematical model and the numerical discretization follow \cite{Stoll1, Stoll} \TODO{cite myself?}. \\
%Let us define $\Omega \subset \mathbb R^n$ an open and bounded regular domain and the time interval $[0,T]$. Let $Y$ and $H$ be two separable Hilbert spaces which verify the Gelfand triple chain $Y \hookrightarrow H \hookrightarrow Y\dual$ and another Hilbert space $U$. 
%Let us define the space and adjoint space as 
%$
%\Cal Y_t := 
%\displaystyle \Big \{
%y \in L^2(0,T; Y)  \;\; \text{s.t.} \;\;  \dt{y} \in L^2(0,T; Y) 
%\Big \}.
%$
%Moreover, the control variable is considered in the space $\Cal U = L^2(0,T; U)$.
%The  general formulation of the \ocp s considered is: given $\pmb \mu \in \mathscr P$, find
%$(y(\bmu), u(\bmu)) \in \Cal Y_t \times \Cal U$ which verify 
%\begin{equation}
%\label{J_functional}
%\min_{(y,u) \in \Cal Y_t \times \Cal U} 
%\frac{1}{2} \intTimeSpace{(y - y_d(\pmb \mu))^2} %+ \frac{\gamma_2}{2} \intSpace{(y(T) - y_T(\pmb \mu))^2} 
%+ \alf \intTimeSpace {u^2}
%\end{equation}
%constrained to the following weak equation
%\begin{equation}
%\label{eq_time_weak}
%\begin{cases}
%\displaystyle \intTime{ \Big \la \dt y, q \Big \ra_{Y\dual, Y}}
%+ \intTime {a (y, q; \bmu)} =
%\intTimeSpace{uq} 
%+\intTime{ \la G(\bmu), q \ra_{Y\dual, Y}} & \forall q \in \Cal Y_t, \\
%y(0) = y_0  & \text{in } \Omega,
%\end{cases}
%\end{equation}
%where $a \goesto{\Cal Y_t}{\Cal  Y_t}{\mathbb R}$ is a bilinear differential state operator and $G \in \Cal Y\dual $ collects forcing and boundary terms of the state operator. Furthermore, we assume $\norm{y_0}_H=0$. Let us define $\Cal X = \Cal Y_t \times \Cal U$ with the norm induced by the product. We exploit a Lagrangian approach, i.e. the minimization problem is solved defining the Lagrangian functional 
%\begin{equation}
%\label{functional}
%\Lg (y,u,p; \bmu) = \half  \Cal A (x,x; \pmb \mu)  - \intTime{\la F(\bmu), x \ra} + \Cal B((y,u), p; \bmu) 
%+ \la G(\bmu), p \ra
%\end{equation} 
%where the bilinear forms are defined as:
%\begin{align*}
%\Cal A \goesto {\Cal X}{\Cal X}{\mathbb R} & \spazio
%\Cal A(x,w) = \intTimeSpace{y,z} +\alpha \intTimeSpace{uv} & 
%\spazio \forall x, w \in \Cal X, \\
%\Cal B \goesto {\Cal X}{\Cal Y_t}{\mathbb R} & \spazio
%\Cal B(w, q; \bmu) = \intTime { \Big \la \dt z , q \Big \ra } + a(z, q; \bmu) - c(v, q; \bmu)& 
%\spazio \forall w \in \Cal X, \forall q \in \Cal Y_t,\\
%F(\bmu) \in \Cal X\dual & \spazio
%\la F(\bmu), w \ra = m(y_d(\bmu),z) & 
%\spazio \forall w\in \Cal X. \\
%\end{align*}
%
%Then, we perform a differentiation by the adjoint variable $p$, the state variable $y$ and the control $u$.
%The minimization of \eqref{functional} is equivalent to find the solution of the following system: given $\pmb \mu \in \mathscr P$, find $(x(\pmb \mu), p(\pmb \mu)) \in \Cal X \times \Cal Y$  
%\begin{equation}
%\label{optimality_system}
%\begin{cases}
%D_y\Lg(y, u, p; \pmb \mu)[z] = 0 & \forall z \in \Cal Y_t,\\
%D_u\Lg(y, u, p; \pmb \mu)[v] = 0 & \forall v \in \Cal U,\\
%D_p\Lg(y, u, p; \pmb \mu) [q]= 0 & \forall q \in \Cal Y_t.\\
%\end{cases}
%\end{equation}

==> references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
%\bibliographystyle{spmpsci}
\bibliography{Bib_Maria}
%
%\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} If the citatiion in the text is numbered, the reference list should be arranged in ascending order. If the citation in the text is author/year, the reference list should be \textit{sorted} alphabetically and if there are several works by the same author, the following order should be used:
%\begin{enumerate}
%\item all works by the author alone, ordered chronologically by year of publication
%\item all works by the author with a coauthor, ordered alphabetically by coauthor
%\item all works by the author with several coauthors, ordered chronologically by year of publication.
%\end{enumerate}
%The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
%\begin{itemize}
%\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
%\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
%\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
%\item Examples of the basic Springer Nature style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
%\end{itemize}
%}
%
%\begin{thebibliography}{99.}%
%% and use \bibitem to create references.
%%
%% Use the following syntax and markup for your references if 
%% the subject of your book is from the field 
%% "Mathematics, Physics, Statistics, Computer Science"
%%
%% Contribution 
%\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%%
%% Online Document
%\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
%\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%%
%% Monograph
%\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%%
%% Journal article
%\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%%
%% Journal article by DOI
%\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%%
%\bigskip
%
%% Use the following (APS) syntax and markup for your references if 
%% the subject of your book is from the field 
%% "Mathematics, Physics, Statistics, Computer Science"
%%
%% Online Document
%\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
%\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%%
%% Monograph
%\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%%
%% Journal article
%\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%%
%% Journal article by DOI
%\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%%
%% Contribution 
%\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%%
%\bigskip
%%
%% Use the following syntax and markup for your references if 
%% the subject of your book is from the field 
%% "Psychology, Social Sciences"
%%
%%
%% Monograph
%\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%%
%% Online Document
%\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
%\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%%
%% Journal article
%\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%%
%% Contribution 
%\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%%
%% Journal article by DOI
%\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%%
%%
%% Use the following syntax and markup for your references if 
%% the subject of your book is from the field 
%% "Humanities, Linguistics, Philosophy"
%%
%\bigskip
%%
%% Journal article
%\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%%
%% Contribution 
%\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%%
%% Monograph
%\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%%
%% Online Document
%\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
%http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%%
%% Journal article by DOI
%\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O'Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%%
%%
%%
%\bigskip
%%
%%
%% Use the following syntax and markup for your references if 
%% the subject of your book is from the field 
%% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%%
%%
%% Contribution 
%\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%%
%% Online Document
%\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
%\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%%
%% Journal article by DOI
%\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%%
%% Journal article
%\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%%
%% Monograph
%\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%%
%\end{thebibliography}

